Small Vision-Language Models Are Fast Self-Checking Pointing Decision Models

Robots, drones and web agents act by pointing, yet vision-language models (VLMs) point by generating coordinate tokens one at a time: each point costs a chain of dependent forward passes, and its token probabilities are only a rough guide to whether it is right. A decision model instead scores every answer in one forward pass and acts on the best one, but today's decision models for grounding choose among coarse options or need a round of questions for each finer level. We show that a VLM that writes coordinates as digits is already an accurate pointing decision model. Each axis has only 111 digit prefixes, all known before anything is generated. Read together as short continuations of the same image and instruction, their next-digit probabilities give each axis a distribution over all its values, and so a probability map on a 1000x1000 grid or any coarser one, with no new head. Off the shelf, this read is as accurate as the generated point and, for Qwen3.5, 2.4 to 2.8 times faster. Fine-tuning then makes the read one pass, by asking each axis as its own question, and more accurate, by training each box as a set that contains the answer rather than as its centre. The same pass also reads a self-check, the model's yes or no on whether it can point precisely. Across twelve VLMs of up to 4B parameters, the resulting model is 1.9 to 4.4 pp more accurate than the same VLM fine-tuned to write its point, and makes fewer confident errors than that model ranked by its own probabilities. To test at on-device speed, we hold each decision to its measured Raspberry Pi 5 time in a drone simulator, where our 0.8B model reaches the most targets; on web tasks, its self-check leaves fewer confident wrong clicks.

==> layout.tex <==
\usepackage[T1]{fontenc}\usepackage{times}   %
\usepackage{varwidth}
\setcitestyle{numbers,square,comma}
\makeatletter
\let\arxivorigvspace\vspace
\newcommand{\arxivfloatvspace}{\@ifstar{\arxivfv}{\arxivfv}}
\newcommand{\arxivfv}[1]{\setlength{\dimen@}{#1}\ifdim\dimen@<\z@\else\arxivorigvspace{#1}\fi}
\newlength{\arxivcolmax}\setlength{\arxivcolmax}{0.62\textwidth}
\newlength{\arxivcapgap}\setlength{\arxivcapgap}{1.8em}
\newsavebox{\arxivfloatbox}
\newif\ifarxivwide
\gdef\arxivwidefrac{1}
\newcommand{\arxivwidenext}[1]{\global\arxivwidetrue\gdef\arxivwidefrac{#1}}
\newcommand{\arxivsideput}{%
  \noindent\begin{minipage}[t]{\wd\arxivfloatbox}\vspace{0pt}\usebox{\arxivfloatbox}\end{minipage}%
  \hfill\begin{minipage}[t]{\dimexpr\textwidth-\wd\arxivfloatbox-\arxivcapgap\relax}\vspace{0pt}%
  \setlength{\abovecaptionskip}{\z@}\setlength{\belowcaptionskip}{\z@}}
\newcommand{\arxivsidebegin}{\let\vspace\arxivfloatvspace
  \ifarxivwide\global\arxivwidefalse
    \centering\begin{minipage}{\arxivwidefrac\textwidth}\centering
  \else
    \let\arxivorigcaption\caption
    \def\caption{\end{varwidth}\end{lrbox}\arxivsideput\arxivorigcaption}%
    \begin{lrbox}{\arxivfloatbox}\begin{varwidth}{\arxivcolmax}\centering
  \fi}
\makeatother
\let\arxivfigure\figure\let\endarxivfigure\endfigure
\let\arxivtable\table\let\endarxivtable\endtable
\renewenvironment{figure}[1][tbp]{\arxivfigure[#1]\arxivsidebegin}{\end{minipage}\par\vskip0pt\endarxivfigure}
\renewenvironment{table}[1][tbp]{\arxivtable[#1]\arxivsidebegin}{\end{minipage}\par\vskip0pt\endarxivtable}
\renewenvironment{figure*}[1][tbp]{\arxivfigure[#1]\let\vspace\arxivfloatvspace}{\endarxivfigure}
\renewenvironment{table*}[1][tbp]{\arxivtable[#1]\let\vspace\arxivfloatvspace}{\endarxivtable}
\setlength{\floatsep}{18pt plus 4pt minus 2pt}\setlength{\textfloatsep}{20pt plus 4pt minus 4pt}   %
\newcount\arxivlooseness\let\looseness\arxivlooseness
\setlength{\emergencystretch}{1.5em}   %

